Can we Retrieve Everything All at Once? ARM: An Alignment-Oriented LLM-based Retrieval Method

Real-world open-domain questions can be complicated, particularly when answering them involves information from multiple information sources. LLMs have demonstrated impressive performance in decomposing complex tasks into simpler steps, and previous work has used it for better retrieval in support of complex questions. However, LLM's decomposition of questions is unaware of what data is available and how data is organized, often leading to a sub-optimal retrieval performance. Recent effort in agentic RAG proposes to perform retrieval in an iterative fashion, where a followup query is derived as an action based on previous rounds of retrieval. While this provides one way of interacting with the data collection, agentic RAG's exploration of data is inefficient because successive queries depend on previous results rather than being guided by the organization of available data in the collection. To address this problem, we propose an LLM-based retrieval method -- ARM, that aims to better align the question with the organization of the data collection by exploring relationships among data objects beyond matching the utterance of the query, thus leading to a retrieve-all-at-once solution for complex queries. We evaluated ARM on two datasets, Bird and OTT-QA. On Bird, it outperforms standard RAG with query decomposition by up to 5.2 pt in execution accuracy and agentic RAG (ReAct) by up to 15.9 pt. On OTT-QA, it achieves up to 5.5 pt and 19.3 pt higher F1 match scores compared to these approaches.

==> sections/limitation.tex <==
\section{Limitations}
First, we wanted to note the limitations of the choice of our evaluation datasets.
Though our retrieval framework with the data representation method in Section~\ref{sec:index} can be applied to different modalities, our experiments mainly focus on text and tables. We defer creating a benchmarking dataset that answering questions requires joint reasoning over text, tables, and images,  and evaluating our method on it as a future work.

Secondly, our method can only work when using open-sourced models. It can not be applied to models that are only accessible through APIs.
